Differentiable Implicit Layers

In this paper, we introduce an efficient backpropagation scheme for non-constrained implicit functions. These functions are parametrized by a set of learnable weights and may optionally depend on some input; making them perfectly suitable as a learnable layer in a neural network. We demonstrate our scheme on different applications: (i) neural ODEs with the implicit Euler method, and (ii) system identification in model predictive control.

==> chapters/dil_particles.tex <==
\subsection{Quasi-Monte Carlo Inference of Neural SDEs by the Stein's Method}
\label{sec:control}
%begin{wrapfigure}{r}{0.25\textwidth}
%    \begin{center}
%		\def\svgwidth{.25\columnwidth}
%		\graphicspath{{sketches/}}
%		{\input{sketches/ensde.pdf_tex}}
%		\caption{ENSDE as an instance of  DIL. }
%		\label{fig:concept_ensde}
%		\vspace{-20pt}
%	\end{center}
%\end{wrapfigure}
%A \textit{goodness of fit test} (GOFT) evaluates a discrepancy measure $\mathbf{D}(p, q)$ between a set of particles $q = \bm x^{(1:P)}$, and a distribution $p(\bm x)$. There are %many different choices for $\mathbf{D}(p, q)$, like Stein discrepancy \citep{goodness_of_fit} or maximum mean discrepancy \citep{smola_mmd}. The GOFT serves as a starting point for %deriving particle methods, which place a set of particles $q$, such that the discrepancy measure $\mathbf{D}(p, q)$ is minimized. Such particle methods are used e.g. for signal %filtering \citep{seq_kernel_herding} or generating super-samples \citep{chen_kherding}. \cite{grathwohl_stein} propose a learning framework for fitting a distribution $p(\bm x)$ to %a set of particles $q$. However, a common problem of these methods is the missing backward evaluation in order to learn a model $p(\bm x)$, such that the generated particles $q$ %exhibit a desired behaviour on a downstream  loss function $\mathcal{L}(q)$. Our framework is able to address this problem. Below, we give an illustrative example when the Stein %discrepancy is chosen as $\mathbf{D}(p, q)$. The same reasoning can be applied to other discrepancy measures.

The kernelized Stein discrepancy $\mathbf{KSD}(p, q)$  \citep{goodness_of_fit} estimates a discrepancy measure between a set of particles $q = \bm x^{(1:P)}$, and a distribution $p(\bm x)$. Together with \textit{Stein variational gradient descent} (SVGD) \citep{stein, stein_flow} $\mathbf{KSD}(p, q)$ can be used to generate high quality samples (particles) from the distribution $p(\bm x)$. Such particle methods are used e.g. for signal filtering \citep{stein_filtering}.
Moreover, \cite{grathwohl_stein} propose a learning framework for fitting a distribution $p(\bm x)$ to a set of particles $q$. However, a common problem of these methods is the missing backward evaluation in order to learn a model $p(\bm x)$, such that the generated particles $q$ exhibit a desired behaviour on a downstream  loss function $\mathcal{L}(q)$. Our framework is able to address this problem. Below, we give an illustrative example.


\paragraph{Equilibrium Neural SDEs (ENSDE).} 
We are interested in sampling from the invariant distribution 
$\lim_{t \rightarrow \infty} p(\bm x, t) = p_\infty (\bm x)$, when dynamics is governed by an autonomous \textit{stochastic differential equation} (SDE)
\citep{sde_numerics}:
\begin{equation*}
    d \bm x = \frac{\partial v(\bm x)}{\partial \bm x} dt + \sqrt{2\epsilon} d \bm w 
    \xrightarrow[Planck-Eq.]{Fokker} \lim_{t \rightarrow \infty} p(\bm x, t)=p_\infty (\bm x) \propto e^{v(\bm x)/\epsilon} , 
\end{equation*}
with $\bm w$ denoting a Wiener process. We assume the drift function of the SDE to be the gradient of a potential. 
For such a process we can derive the invariant distribution $p_\infty(\bm x)$ in closed form, as we  detail in Appx. \ref{app:invariant}.  
When replacing the drift function of the SDE by a neural network, i.e. $\nicefrac{\partial v(\bm x)}{\partial \bm x}=\bm h(\bm x; \bm \theta)$, we
obtain a \textit{neural SDE} (NSDE) \citep{nsde_limit, dbnn}. 
We refer to such a NSDE as an {\it Equilibrium NSDE} (ENSDE), since it can be regarded as a stochastic extension to \textit{Deep Equilibrium Models} \citep{deepeq}, 
which estimates an output as an infinitely often evaluation with a deterministic network.
Similarly, we could pass an input infinitely often through the corresponding NSDE, instead of sampling from $p_\infty(\bm x)$. 
However directly sampling a set of particles $q$ from $p_\infty(\bm x; \bm \theta)$ is more favourable.
We infer the set of particles $q$ as an $\argmin$-solution to the \textit{kernelized Stein discrepancy} $\mathbf{KSD}(p_\infty(\bm x; \bm \theta), q)$ \citep{goodness_of_fit}:
\begin{equation}
    \argmin_{q=x^{(1:P)}}\mathbf{KSD}(p_\infty(\bm x; \bm \theta), q)= \argmin_{q=x^{(1:P)}} \frac{1}{P^2} \sum_{i,j=1}^{P} \bm s^T \kappa \bm s 
    + \bm s^T \frac{\partial \kappa}{\partial \bm x_j} + \frac{\partial \kappa}{\partial \bm x_j}^T \bm s
    +  \text{tr}\big({\frac{\partial^2 \kappa }{\partial \bm x_i \partial \bm x_j}}\big),
    \label{eq:ksd}
\end{equation}
with $\bm s(\bm x)= \nicefrac{\partial \log p_\infty(\bm x; \bm \theta)}{\partial \bm x}=\nicefrac{\bm h(\bm x; \bm \theta)}{\epsilon}$ and the  kernel 
$\kappa(\cdot, \cdot)$. 
We obtain an efficient evaluation procedure for $\mathbf{KSD}(p_\infty(\bm x; \bm \theta),q)$, since the costly to evaluate term $\bm s(\bm x)$ is 
the scaled drift of the NSDE, i.e. $\nicefrac{\bm h(\bm x; \bm \theta)}{\epsilon}$.
We minimize the $\mathbf{KSD}(p_\infty(\bm x; \bm \theta),q)$  with the commonly used 
SVGD. 
Consequently, $\mathbf{KSD}(p_\infty(\bm x; \bm \theta),q)$ can be treated as the score function $f$ and SVGD as the $\texttt{solver}$ in our proposed framework. 
\newpage
\begin{wrapfigure}{r}{0.4\textwidth}
    \begin{center}
	    \centering
	    \includegraphics[height=.25\columnwidth]{pix/dynamics_deepeq_nsde.pdf}
		\caption{Dynamics of trained NSDE.}
		\label{fig:deepeq_dyn}
		%\vspace{-20pt}
	\end{center}
\end{wrapfigure}


%\begin{figure}[h]
%    \centering
%    \begin{minipage}{0.48\textwidth}
%	    \centering
%	    \includegraphics[height=.5\columnwidth]{pix/dynamics_deepeq_nsde.pdf}
%		\caption{Dynamics of trained NSDE.}
%		\label{fig:deepeq_dyn}
 %   \end{minipage}\hfill
  %  \begin{minipage}{0.48\textwidth}
%	    \centering
%	    \includegraphics[height=.5\columnwidth]{pix/svgd_deepeq_nsde.pdf}
%	    \caption{Sampling from $\lim_{t \rightarrow \infty} p(\bm x, t)$.}
%		\label{fig:deepeq_svgd}
 %   \end{minipage}
%\end{figure}

\paragraph{ENSDE Training.} 
We train the ENSDE by minimizing a loss function $\mathcal{L}(q)$ that depends on the particles $q$. We fix the number of particles to 32. 
The loss function is the $\mathbf{KSD}$ between the particles $q$ and the reference distribution $p_{\infty}^{ref}(\bm x)=\nicefrac{\mu- \bm x}{\epsilon}$, with $\mu=2$ and $\epsilon=0.05$, which 
amounts to an Ornstein-Uhlenbeck process. We express the training objective as a nested $\argmin$-problem: 
\begin{equation*}
     \argmin_{\theta}\mathbf{KSD}(p_{\infty}^{ref}(\bm x),  \argmin_{q=x^{(1:P)}}\mathbf{KSD}(p_\infty(\bm x; \bm \theta), q)).
\end{equation*}
As expected, the trained equilibrium NSDE matches the target distribution for $t \rightarrow \infty$ (here from $\sim 10\,s$ 
onwards), satisfying the proof of concept. Naturally, it may miss the intermediate steps.
Fig. \ref{fig:deepeq_dyn} visualizes the learned dynamics of an equilibrium NSDE (architecture in Appx. \ref{app:architect}) for different initial positions. 
As shown in Fig. \ref{fig:deepeq_svgd} SVGD generates high quality samples from $p_\infty(\bm x; \bm \theta)$ after 16 steps, 
instead of integrating the NSDE up to a minimal time of $10\,s$.







==> chapters/intro_legacy.tex <==
\section{Introduction}
\label{sec:intro}

Dynamical systems are often described by an ordinary differential equation (ODE). 
Motivated by this, neural ODEs (NODEs) \citep{neural_ode} are a natural design choice for dynamical systems modeling.
Research on NODEs involves learning of second order dynamics \citep{odevae}, time evolving weights \citep{anode_v2, davis2020time}, proper regularization techniques \citep{node_regular}, as well as discussion about their theoretical properties \citep{aug_ode, dissect_ode}.
However NODEs suffer from several pain points: (i) inconsistent gradient estimation, (ii) high run time during training, and (iii) missing capability for stiff system identification. 
Using the adjoint training method \citep{neural_ode} is well known to cause numerical instabilities, due to non reversibility of NODEs \citep{anode}. 
Further the adjoint method requires during the backward pass an additional computational costly solution to the induced ODE problem. 
Lastly current NODEs rely on explicit solvers or semi-implicit methods only, which lack numerical stability guarantees. 
We address all of these points by following contributions:
\begin{itemize}
\item Motivated by implicit solvers for ODEs, we introduce the \textit{Backward Euler NODE} (BENODE). 
Using the backward Euler solver comes with bigger numerical stability regions compared to explicit solvers for NODEs. 
\item We propose different iterative and analytical solution methods to the implicit problem induced during the forward
propagation of BENODEs. 
\item We introduce a novel training method based on the inverse function theorem (IFT). Using IFT comes with the benefit of (i) beeing potentially faster and (ii) having zero gradient error compared to the alternative adjoint method \citep{neural_ode}.
\end{itemize}
We demonstrate on a number of different tasks superior behaviour in terms of training time and prediction accuracy of our novel method.


